Post-Newtonian Jeans analysis

The Jeans analysis is studied in the first post-Newtonian limit. In other words, the relativistic effects on the local gravitational instability are considered for systems where characteristic velocity of the system and corresponding gravitational field are higher than what permitted in Newtonian limit. The dispersion relation for propagation of small perturbations is found in the post-Newtonian approximation using two different techniques. A new Jeans mass is derived and compared to the standard Jeans mass. In this limit, the relativistic effects make the new Jeans mass to be smaller than the Newtonian Jeans mass. Furthermore, the fractional difference between these two masses increases when temperature/pressure of the system increases. Interestingly, in this limit pressure can help the gravitational instability instead of preventing it. Finally the results are applied to high temperature astrophysical systems and the possibility of local fragmentations in some relativistic systems is investigated.

==> Ref.tex <==

\begin{thebibliography}{}


\bibitem{} Anderson, L. D., Bania, T. M., Jackson, J. M., Clemens, D. P., Heyer, M., Simon, R., ... \& Rathborne, J. M., 2009, The Astrophysical Journal Supplement Series, 181, 1
\bibitem{} Binney, J. \& Tremaine, S., Galactic dynamics, 2011, Princeton university press
\bibitem{} Blandford R. \& Teukolsky S. A., 1969, Astrophys. J., 205, 55
\bibitem{} Boss, A. P., \& Sandra A. K. 2010, The Astrophysical Journal Letters, 717, L1
\bibitem{} Burke W. L.,1971, J. Math. Phys., 401
\bibitem{} Chandrasekhar, S. , 1967, Astrophys. J., 148, 621
\bibitem{} Chandrasekhar, S. \&  Nutku, Y., 1969, Astrophys. J., 158, 55
\bibitem{} Chandrasekhar, S. \& Esposito, F. P., 1970, Astrophys. J., 160, 153
\bibitem{} Chandrasekhar, S., 1965, Astrophys. J., 142, 1488
\bibitem{} Chandrasekhar, S.,1969 ,Astrophys. J., 158, 45
\bibitem{} Damour, T., \& Taylor, 1991, J. H., Astrophys. J., 366 , 501
\bibitem{} Demianski, M.\& Ivanov, P. B., 1997, Astronomy and Astrophysics, 324, 829
\bibitem{} Einstein, A., 1915, Preuss. Akad. Wiss. Berlin, 47, 831
\bibitem{} Epstein, R., 1977, Astrophys. J., 216, 92
\bibitem{} Faber, J. A., \& Rasio, F. A., 2000, Physical Review D, \textbf{62}, 6
\bibitem{} Guobin, M.,  et al., 2014,  The Astrophysical Journal, 790.2, 109
\bibitem{} Hulse, R. A. \& Taylor, J. H., 1975, Astrophys. J. Lett., 195, L51
\bibitem{} Kastner, J. H., et al., 2002, The Astrophysical Journal, 672.2, 957
\bibitem{} Kastner, J. H., Montez Jr, R., Balick, B., \& De Marco, O., 2008, The Astrophysical Journal, 672, 2
\bibitem{} Kimura, M., Tsunemi, H., Tomida, H., Sugizaki, M., Ueno, S., Hanayama, T., ... \& Sasaki, M. (2013). Publications of the Astronomical Society of Japan, 65(1), 14.
\bibitem{} Kohri, K., \&  Mineshige S., 2002, The Astrophysical Journal, 577.1, 311
\bibitem{} Lai, D., \& Wiseman, A. G., 1996, Physical Review D, 54, 6
\bibitem{} Latter, W. B., et al., 2000,  The Astrophysical Journal 539.2, 783
\bibitem{} Levenson, N. A., Graham, J. R., Aschenbach, B., Blair, W. P., Brinkmann, W., Busser, J. U., ... \& Klein, R. I. (1997), The Astrophysical Journal, 484(1)
\bibitem{} Masaru S., et al., 2006, Physical review letters, 96.3, 031102
\bibitem{} Masashi, K.,  et al., 2013, Publications of the Astronomical Society of Japan, 65.1, 14
\bibitem{} Masson, C. R. (1989). The Astrophysical Journal, 336
\bibitem{} Marcolino, W. L. F., Hillier, D. J., De Araujo, F. X., \& Pereira, C. B. (2007). The Astrophysical Journal, 654(2).
\bibitem{} Mo, H., Van den Bosch, F., White, S., 2010, Galaxy formation and evolution, Cambridge University Press 
\bibitem{} Mou, G., Yuan, F., Bu, D., Sun, M., \& Su, M. (2014). The Astrophysical Journal, 790(2), 109.
\bibitem{} Mufson, S. L., Lyon, J., \& Marionni, P. A. (1975). The Astrophysical Journal, 201
\bibitem{} Poisson, E. \& Will, C. M., 2014, Gravity: Newtonian, Post-Newtonian, Relativistic, Cambridge University Press
\bibitem{} Rezzolla, L. \& Zanotti O., Relativistic hydrodynamics, Oxford University Press
\bibitem{} Ruiz, N., et al., 2013, The Astrophysical Journal, 767.1, 35
\bibitem{} Will, C. M., in 300 Years of Gravitation, ed. S. Hawking and W. Israel, 1987, Cambridge, 80
\bibitem{} Will, C. M., in Proceedings of the Eighth Nishinomiya- Yukawa Memorial Symposium on Relativistic Cosmology, ed. M. Sasaki (Tokyo, 1994, Universal Academy Press)
\bibitem{} Will, C. M., 2011, PNAS, 108, 15
\bibitem{} Zhekov, S. A., \& M. Perinotto., 1996, Astronomy and Astrophysics, 309, 648

\bibitem{} Kim, W.-T., \& Ostriker, E. C. 2001, ApJ, 559, 70
\bibitem{} Toomre, A. 1964, ApJ, 139, 1217
\bibitem{} Vandervoort, P. O. 1970, ApJ, 161, 87
\bibitem{} Kato, S. 1972, PASJ, 24, 61
\bibitem{} Rafikov, R. R. 2001, MNRAS, 323, 445
\bibitem{} Romeo, A. B. 1992, MNRAS, 256, 307
\bibitem{} Romeo, A. B., \& Wiegert, J. 2011, MNRAS, 416, 1191
\bibitem{} Bertin, G., \& Romeo, A. B. 1988, A\&A, 195, 105
\bibitem{} Shadmehri M., Khajenabi F., 2012, MNRAS, 421, 841
\bibitem{} Jog, C. J., \& Solomon, P. M. 1984, ApJ, 276, 114
\bibitem{} Jog, C. J. 1996, MNRAS, 278, 209

\bibitem{} Elmegreen, B. G. 1987, ApJ, 312, 626
\bibitem{} Elmegreen, B. G. 1995, MNRAS, 275, 944
\bibitem{} Elmegreen, B. G. 2011, ApJ, 737, 1
\bibitem{} Gammie, C. F. 1996, ApJ, 462, 725
\bibitem{} 
  J.~Freundlich, C.~J.~Jog and F.~Combes,
  %``Local stability of a gravitating filament: a dispersion relation,''
  Astron.\ Astrophys.\  {\bf 564}, A7 (2014)
\bibitem{} 
  M.~Roshan and S.~Abbassi,
  %``Jeans analysis in modified gravity,''
  Phys.\ Rev.\ D {\bf 90}, no. 4, 044010 (2014)  
  \bibitem{}
  M.~Roshan and S.~Abbassi,
  %``On the stability of a galactic disk in modified gravity,''
  Astrophys.\ J.\  {\bf 802} (2015) no.1,  9
  \bibitem{} 
  M.~Roshan and S.~Abbassi,
  %``Local stability of self-gravitating disks in $f(R)$ gravity,''
  Astrophys.\ Space Sci.\  {\bf 358}, no. 1, 11 (2015)
  
  \bibitem{}
S.~Capozziello, M.~De Laurentis, I.~De Martino, M.~Formisano and S.D.~Odintsov, Phys.\ Rev. \ D {\bf 85}, 044022 (2012).

\bibitem{}
  L.~Blanchet,
  %``Gravitational radiation from post-Newtonian sources and inspiralling compact binaries,''
  Living Rev.\ Rel.\  {\bf 9} (2006) 4.
  \bibitem{} 
  C.~M.~Will,
  %``The Confrontation between general relativity and experiment,''
  Living Rev.\ Rel.\  {\bf 9}, 3 (2006)
  \bibitem{} 
  C.~J.~Jog,
  Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 434}, 56 (2013) 
  \bibitem{} 
  D.~M.~Siegel, R.~Ciolfi, A.~I.~Harte and L.~Rezzolla,
  Phys.\ Rev.\ D {\bf 87}, no. 12, 121302 (2013)
    \bibitem{} 
  Blandford R. D., Pringle J. E., 1976, MNRAS, 176, 443
    \bibitem{} 
  Ferrari A., Trussoni E., Zaninetti L., 1978, A\& A, 64, 43
  \bibitem{} 
  Zhang B., MacFadyen A., Wang P., 2009, ApJ, 692, L40
  \bibitem{} 
  Hardee P. E., Norman M. L., 1988, ApJ, 334, 70
\end{thebibliography}
